Efficient lossless coding of highpass bands from block-based motion compensated wavelet lifting using JPEG 2000

Lossless image coding is a crucial task especially in the medical area, e.g., for volumes from Computed Tomography or Magnetic Resonance Tomography. Besides lossless coding, compensated wavelet lifting offers a scalable representation of such huge volumes. While compensation methods increase the details in the lowpass band, they also vary the characteristics of the wavelet coefficients, so an adaption of the coefficient coder should be considered. We propose a simple invertible extension for JPEG 2000 that can reduce the filesize for lossless coding of the highpass band by 0.8% on average with peak rate saving of 1.1%.

==> tab/tabentries-praes.tex <==
 \it{heart spat} & 98 880 861 & \textbf{97 776 086} & \textbf{97 776 578} &  1 104 775 &  1 104 283 &  -0.045  \tabularnewline 
 \it{heart time} & 92 972 210 & \textbf{92 122 327} & \textbf{92 122 485} &  849 883 &  849 725 &  -0.019  \tabularnewline 
 \it{head} & \textbf{3 751 832} & 3 751 834 & 3 751 834 &  -2 &  -2 &  0  \tabularnewline 
 \it{head 2} & \textbf{7 318 102} & 7 318 107 & 7 318 107 &  -5 &  -5 &  0  \tabularnewline 
 \it{head 3} & 1 502 434 & \textbf{1 492 997} & \textbf{1 493 900} &  9 437 &  8 534 &  -9.569  \tabularnewline 
 \it{head 4} & 1 814 188 & \textbf{1 809 398} & \textbf{1 811 464} &  4 790 &  2 724 &  -43.132  \tabularnewline 
 \it{thorax 1} & 7 661 846 & \textbf{7 651 164} & \textbf{7 651 651} &  10 682 &  10 195 &  -4.559  \tabularnewline 
 \it{thorax 2} & \textbf{5 979 688} & 5 979 693 & 5979 693 &  -5 &  -5 &  0  \tabularnewline 
 \it{thorax 3} & \textbf{7 850 487} & 7 850 492 & 7850 492 &  -5 &  -5 &  0  \tabularnewline 
 \it{thorax 4} & 9 164 221 & \textbf{9 163 155} & \textbf{9 163 335} &  1 066 &  886 &  -16.886  \tabularnewline 

